Higher order mixed moment approximations for the Fokker-Planck equation in one space dimension

We study mixed-moment models (full zeroth moment, half higher moments) for a Fokker-Planck equation in one space dimension. Mixed-moment minimum-entropy models are known to overcome the zero net-flux problem of full-moment minimum entropy Mn models. Realizability theory for these mixed moments of arbitrary order is derived, as well as a new closure, which we refer to as Kershaw closures. They provide non-negative distribution functions combined with an analytical closure. Numerical tests are performed with standard first-order finite volume schemes and compared with a finite-difference Fokker-Planck scheme.

==> Images/1Beam/1Beam.tex <==
\left(\begin{array}{ccccccc} \mathrm{Model} & \mathrm{L1} & \mathrm{L2} & \mathrm{Linf} & \mathrm{CL1} & \mathrm{CL2} & \mathrm{CLinf}\\ \mathrm{MM1} & 0.066339 & 0.033333 & 0.099496 & 0.01773 & 0.022299 & 0.041594\\ \mathrm{MK1} & 0.16669 & 0.071425 & 0.21744 & 0.049446 & 0.053638 & 0.075535\\ \mathrm{M1} & 0.07234 & 0.033757 & 0.11092 & 0.020511 & 0.023531 & 0.050847\\ \mathrm{MK2} & 0.10197 & 0.04527 & 0.19809 & 0.033389 & 0.037324 & 0.052803\\ \mathrm{FP} & 0 & 0 & 0 & 0 & 0 & 0\\ \mathrm{P3} & 0.074409 & 0.042993 & 0.21298 & 0.01355 & 0.017695 & 0.035565\\ \mathrm{P7} & 0.042149 & 0.022403 & 0.0851 & 0.015638 & 0.020247 & 0.049295\\ \mathrm{P13} & 0.02321 & 0.012092 & 0.033303 & 0.0087753 & 0.011564 & 0.022437\\ \mathrm{P51} & 0.0059108 & 0.0026413 & 0.0055583 & 0.0023004 & 0.002608 & 0.0050124 \end{array}\right)

==> Images/2Beams/2Beams.tex <==
\left(\begin{array}{ccccccc} \mathrm{Model} & \mathrm{L1} & \mathrm{L2} & \mathrm{Linf} & \mathrm{CL1} & \mathrm{CL2} & \mathrm{CLinf}\\ \mathrm{MA1} & 0.010005 & 0.10002 & 0.0025472 & 0.0025031 & 0.0025032 & 0.0025102\\ \mathrm{MA2} & 0.009977 & 0.10001 & 0.0044977 & 0.0024997 & 0.0025043 & 0.0027055\\ \mathrm{MME} & 0.014096 & 0.12361 & 0.0055959 & 0.0038968 & 0.0042576 & 0.0055318\\ \mathrm{MP3} & 0.66246 & 1.1237 & 1.9032 & 0.13701 & 0.30162 & 1.8886\\ \mathrm{MP2} & 1.0014 & 1.2666 & 2.0879 & 0.22026 & 0.38489 & 2.087\\ \mathrm{MP5} & 0.37857 & 0.93348 & 1.5572 & 0.071395 & 0.20711 & 1.5519\\ \mathrm{P5} & 0.32975 & 0.65532 & 0.29795 & 0.062191 & 0.09103 & 0.23609\\ \mathrm{MP10} & 0.14579 & 0.66405 & 0.9418 & 0.023389 & 0.10519 & 0.93944\\ \mathrm{P11} & 0.14739 & 0.47281 & 0.16725 & 0.025458 & 0.047333 & 0.16291\\ \mathrm{P21} & 0.064425 & 0.34534 & 0.12362 & 0.010751 & 0.025912 & 0.12202\\ \mathrm{K1} & 0.51042 & 0.7974 & 0.25725 & 0.15275 & 0.1857 & 0.21545\\ \mathrm{M1} & 0.57247 & 0.84034 & 0.32016 & 0.16529 & 0.20017 & 0.26776\\ \mathrm{P51} & 0.022045 & 0.21629 & 0.068403 & 0.0046509 & 0.010863 & 0.067418\\ \mathrm{FP} & 0 & 0 & 0 & 0 & 0 & 0\\ \mathrm{M1} & 0.53439 & 0.82276 & 0.25789 & 0.16074 & 0.19928 & 0.21276 \end{array}\right)

==> Images/Sourcebeam/Sourcebeam.tex <==
\left(\begin{array}{ccccc} \mathrm{Model} & \mathrm{AE} & \mathrm{RE} & \mathrm{CAE} & \mathrm{CRE}\\ \mathrm{MME} & 0.19588 & 0.10821 & 0.1072 & 0.10897\\ \mathrm{MK1} & 0.19874 & 0.10979 & 0.10602 & 0.10777\\ \mathrm{MK2} & 0.05301 & 0.029284 & 0.032921 & 0.033466\\ \mathrm{M1} & 0.4961 & 0.27406 & 0.26494 & 0.26932\\ \mathrm{MP10} & 0.16744 & 0.092499 & 0.096714 & 0.098315\\ \mathrm{P21} & 0.05776 & 0.031908 & 0.029278 & 0.029763 \end{array}\right)
